Generalization of the Kuramoto model to the Winfree model by a symmetry breaking coupling

We construct a nontrivial generalization of the paradigmatic Kuramoto model by using an additional coupling term that explicitly breaks its rotational symmetry resulting in a variant of the Winfree Model. Consequently, we observe the characteristic features of the phase diagrams of both the Kuramoto model and the Winfree model depending on the degree of the symmetry breaking coupling strength for unimodal frequency distribution. The phase diagrams of both the Kuramoto and the Winfree models resemble each other for symmetric bimodal frequency distribution for a range of the symmetry breaking coupling strength except for region shift and difference in the degree of spread of the macroscopic dynamical states and bistable regions. The dynamical transitions in the bistable states are characterized by an abrupt (first-order) transition in both the forward and reverse traces. For asymmetric bimodal frequency distribution, the onset of bistable regions depends on the degree of the asymmetry. Large degree of the symmetry breaking coupling strength promotes the synchronized stationary state, while a large degree of heterogeneity, proportional to the separation between the two central frequencies, facilitates the spread of the incoherent and standing wave states in the phase diagram for a low strength of the symmetry breaking coupling. We deduce the low-dimensional equations of motion for the complex order parameters using the Ott-Antonsen ansatz for both unimodal and bimodal frequency distributions. We also deduce the Hopf, pitchfork, and saddle-node bifurcation curves from the evolution equations for the complex order parameters mediating the dynamical transitions. Simulation results of the original discrete set of equations of the generalized Kuramoto model agree well with the analytical bifurcation curves.

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

	\bibitem{tstp2017} T. Stankovski,  T. Pereira,  Peter V. E. McClintock and A. Stefanovska,  \textit{Coupling functions: Universal insights into dynamical interactionmechanisms},
Rev. Mod. Phys. {\bf 89} 045001  (2017).
\bibitem{akev2013} A. Koseska, E. Volkov and J. Kurths,  \textit{Transition from Amplitude  to Oscillation Death Via Turing Bifurcation},  Phys. Rev. Lett. {\bf 111}, 024103 (2013).
\bibitem{zamk2014} A. Zakharova, M. Kapeller, and E. Sch\"oll,  \textit{Chimera Death: Symmetry Breaking in Dynamical Networks}, Phys. Rev. Lett. {\bf 112}, 154101 (2014).
\bibitem{tb2015} T Banerjee,  \textit{Mean-field-diffusion?induced chimera death state}, EuroPhys. . Lett. {\bf 110}, 69993 (2015).
\bibitem{kpvkc2015} K. Premalatha, V. K. Chandrasekar, M. Senthilvelan, and M. Lakshmanan, \textit{Impact of symmetry breaking in networks of globally coupled oscillators},
Phys. Rev. E {\bf 91}, 052915 (2015).
\bibitem{ismk2015} I. Schneider, M. Kapeller, S Loss, A. Zakharova, B. Fiedler and E. Sch\"oll,  \textit{Stable and transient multicluster oscillation death in nonlocally coupled networks}, 
Phys. Rev. E {\bf 92}, 052915 (2015).
\bibitem{kpvkc2016} K. Premalatha, V. K. Chandrasekar, M. Senthilvelan, and M. Lakshmanan, \textit{Different kinds of chimera death states in nonlocally coupled oscillators},
Phys. Rev. E {\bf 93}, 052213 (2016).
\bibitem{wei2017} Wei Zou, Meng Zhan, and J. Kurths, \textit{The impact of propagation and processing delays on amplitude and
	oscillation deaths in the presence of symmetry-breaking coupling}, Chaos {\bf 27}, 114303 (2017).
\bibitem{usks2020} Uday Singh, K. Sathiyadevi, V. K. Chandrasekar, W. Zou, J. Kurths and D. V. Senthilkumar, 
\textit{Trade-off between filtering and symmetry breaking mean-field coupling in inducing macroscopic dynamical states}, New J. Phys. {\bf 22} 093024 (2020).
\bibitem{rkrr2007} R. Karnatak, R. Ramaswamy, and A. Prasad,
{\it Amplitude death in the absence of time delays in identical coupled oscillators}, Phys. Rev. E {\bf 76}, 035201(R) (2007).
\bibitem{amit2012}Amit Sharma amd Manish Dev Shrimali {\it Amplitude death with mean-fild diffusion}, Phys. Rev. E {\bf 85}, 057204 (2012).
\bibitem{wei2022} Wei Zou, S. He , and C. Yao,
{\it Stability of amplitude death in conjugate-coupled nonlinear oscillator networks}, Appl. Math. Lett.  {\bf 131}, 108052 (2022).

\bibitem{w:1}
A. T. Winfree, {\it Biological Rhythms and the Behaviour of Populations of Coupled Oscillators}, J. Theor. Biol. {\bf 16}, 15 (1967).
\bibitem{w:2}
A. T. Winfree, \textit{The Geomentry of Biological Time} (Springer, New York, 1980).

\bibitem{In2}
J. Buck, {\it Synchronous Rhythmic Flashing of Fireflies II}, Quart. Rev. Biol. {\bf
	63}, 265-289 (1988).
\bibitem{In7} Z. N\'eda, E. Ravasz, T. Vicsek, Y. Brechet, and A. L. Barabasi,
{\it Physics of the rhythmic applause}, Phys. Rev. E {\bf 61}, 6987 (2000).


\bibitem{Kuramoto:1984}Y. Kuramoto, \textit{Chemical Oscillations, Waves
	and Turbulence} (Springer, Berlin, 1984).
\bibitem{Acebron:2005}J. A. Acebron, L. L. Bonilla, C. J. P. Vicente, F.
Ritort and R. Spigler, \textit{The Kuramoto model: a
	simple paradigm for synchronization phenomena}, Rev. Mod. Phys. {\bf
	77}, 137 (2005).
\bibitem{In1} A. Pikovsky, M. Rosenblum, and J. Kurths, {\it Synchronization: A
	Universal Concept in Nonlinear Science}(Cambridge University Press, Cambridge, 2001).
\bibitem{In3} C. S. Peskin, {\it Mathematical Aspects of Heart Physiology}
(Courant Institute of Mathematical Sciences, New York, 1975).
\bibitem{In6} S. P. Benz and C. J. Burroughs,{\it Coherent emission from two-dimensional Josephson junction arrays}, Appl. Phys. Lett. {\bf58},
2162 (1991).
\bibitem{In8} M. Rohden, A. Sorge, M. Timme, and D. Witthaut, {\it Self Organized Synchronization in Decentralized Power Grids},
Phys. Rev. Lett. {\bf109}, 064101 (2012).
\bibitem{In10}V. K. Chandrasekar, M. Manoranjani, and Shamik Gupta {\it Kuramoto model in the presence of additional interactions that break rotational symmetry}, Phys.
Rev. E {\bf102}, 012206 (2020).
\bibitem{w1} R. Gallego, E. Montbrio, and D. Pazo, \textit{Synchronization scenarios in the Winfree model of coupled oscillators}, Phys. Rev. E \textbf{96}, 042208 (2017).
\bibitem{w2}Joel T. Ariaratnam, and S. H. Stroatz, \textit{Phase diagram for the Winfree model of coupled nonlinear oscillators}, Phys. Rev. Lett. \textbf{86}, 19 (2001).

\bibitem{w3} F. Giannuzzi, D. Marinazzo, G. Nardulli, M. Pellicoro,
and S. Stramalia,\textit{ Phase diagram of a generalized Winfree model}, Phys. Rev. E \textbf{75}, 051104 (2007).
\bibitem{w4}D. Pazo, and E. Montbrio, \textit{Low-dimensional dynamics of populations of pulse-coupled oscillators}, Phys. Rev. X \textbf{4}, 011009
(2014).
\bibitem{Ott:2008}E. Ott and T. M. Antonsen, \textit{Low dimensional
	behavior of large systems of globally coupled oscillators}, Chaos {\bf 18}, 037113
(2008).
\bibitem{Ott:2009}E. Ott and T. M. Antonsen, \textit{Long time evolution of phase oscillator systems}, Chaos {\bf 19}, 023117
(2009).
\bibitem{ref1}S. Takagi, T. Ueda, \textit{Emergence and transitions of dynamic patterns of thickness oscillation of the plasmodium of the true slime mold Physarum polycephalum}, Physica D \textbf{237}, 420 (2008).
\bibitem{ref2}Y. Murakami, H. Fukuta, \textit{Stability of a pair of planar counter-rotating vortices in a rectangular box}, Fluid Dyn. Res. \textbf{31}, 1 (2002).
\bibitem{ref3}H. Fukuta, Y. Murakami, \textit{Vortex merging, oscillation, and quasiperiodic structure in a linear array of elongated vortices}, Phys. Rev. E \textbf{57}, 449 (1998).
\bibitem{ref4}P. Meunier, T. Leweke, \textit{Elliptic instability of a co-rotating vortex pair}, J. Fluid. Mech. \textbf{533}, 125 (2005).
\bibitem{ref5}K. Czolczynski, P. Perlikowski, A. Stefanski, T. Kapitaniak, \textit{ Synchronization of pendula rotating in different directions}, Commun. Nonlin. Sci. Num. Simul. \textbf{17}, 3658 (2012).
\bibitem{ref6}M. Kapitaniak, K. Czolczynsk, P. Perlikowski, A. Stefanski, T. Kapitaniak, \textit{Synchronous states of slowly rotating pendula}, Phys. Rep. \textbf{541}, 1 (2014).
\bibitem{ref7}K. Czolczynski, P. Perlikowski, A. Stefanski, T. Kapitaniak, \textit{Synchronization of slowly rotating pendulums}, Int. J. Bifurc. Chaos \textbf{22}, 1250128 (2012).
\bibitem{ref8}G.N. Throumoulopoulos, H. Tasso, \textit{Magnetohydrodynamic counter-rotating vortices and synergetic stabilizing effects of magnetic field and plasma flow}, Phys. Plasmas \textbf{17}, 032508 (2010).
\bibitem{ref9}K.T. Kapale, J.P. Dowling, \textit{Vortex phase qubit: Generating arbitrary, counterrotating, coherent superpositions in Bose-Einstein condensates via optical angular momentum beams}, Phys. Rev. Lett. \textbf{95}, 173601 (2005).
\bibitem{ref10}S. Thanvanthri, K. T. Kapale, and J. P. Dowling, \textit{Arbitrary coherent superpositions of quantized vortices in Bose-Einstein condensates via orbital angular momentum of light}, Phys. Rev. A
\textbf{77}, 053825 (2008).
\bibitem{ref11}K. Sathiyadevi, V. K. Chandrasekar, and M. Lakshmanan, \textit{Emerging chimera states under nonidentical counter-rotating oscillators}, Phys. Rev. E \textbf{105}, 034211 (2022).
\bibitem{ref12}M. Tabor, \textit{Chaos and Integrability in Nonlinear Dynamics: An
	Introduction} (John Wiley and Sons, New York, 1988).
\bibitem{gallego}
R. Gallego, E.~Montbrio, and D. Pazo, Phys. Rev. E {\bf 96}, 042208 (2017).
\bibitem{ssyk1986} S. Shinomoto, and Y. Kuramoto,  Prog. Theor. Phys.  {\bf 75}, 1105 (1986).
\bibitem{xpp}B. Ermentrout, \textit{Simulating, Analyzing, and Animating Dynamical Systems: A Guide
	to XPPAUT for Researchers and Students } (Society for Industrial \& Applied Math,
Philadelphia, PA, 2002).
\bibitem{rr1}G. Filatrella, N. F. Pedersen,and K. Wiesenfeld, \textit{Generalized coupling in the Kuramoto model}, Phys. Rev. E \textbf{75}, 017201 1-4 (2007).
\bibitem{rr3}G.Filatrell, N. F. Pedersen, and K. Wiesenfeld, \textit{Generalized coupling in the Kuramoto model}, Phys. Rev. E \textbf{75}, 017201 1–4 (2007).
\bibitem{rr4} D. Pazo, \textit{Thermodynamic limit of the first-order phase transition in the Kuramoto model}, Phys. Rev. E \textbf{72}, 046211 1–6 (2005).
\bibitem{rr5}J. Gomez-Gardenes, S. Gomez, A. Arenas, and Y. Moreno, \textit{Explosive synchronization transitions in scale-free networks}, Phys. Rev.
Lett. \textbf{106}, 128701 1–4 (2011).
\bibitem{rr6} M. K. S. Yeung, and  S. H. Strogatz, \textit{Time delay in the Kuramoto model of coupled oscillators}, Phys. Rev. Lett. \textbf{82}, 648 1–4 (1999).
\bibitem{rr7} O. Mishima, L. D. Calvert and E.  Whalley, \textit{'Melting ice'I at 77 K and 10 kbar: A new method of making amorphous solids}, Nature
\textbf{310}, 393-395 (1984)
\bibitem{rr8} S. Aasland, and P.F. McMillan, \textit{Density-driven liquid–liquid phase separation in the system AI2O3–Y2O3}, Nature  \textbf{369}, 633-636 (1994)
\bibitem{rr9} H. Sanaka, R. Kurita, and H. Mataki, \textit{Liquid-liquid transition in the molecular liquid triphenyl phosphite}, Phys. Rev. Lett. \textbf{92},
025701 (2004)
\bibitem{rr10}I. Jonas, F. Yang and A. Meyer, \textit{Long-range mass transport during structural transitions in metallic glass-forming melts}, Phys. Rev. Lett. \textbf{123}, 055502 (2019).
\bibitem{rr11}S. T. Chui, \textit{Grain-boundary theory of melting in two dimensions}, Phys. Rev. Lett. \textbf{48}, 933 (1982)
\bibitem{rr13}F. Hellmann, P. Schultz, C. Grabow, J. Heitzig, and J. Kurths, \textit{Survivability of deterministic dynamical systems}, Sci. Rep. \textbf{6}, 29654 (2016).
\bibitem{rr14}C. Mitra, A. Choudhary, S. Sinha, J. Kurths, and R. V. Donner, \textit{Multiple-node basin stability in complex dynamical networks}, Phys. Rev. E \textbf{95}, 032317 (2017).
\bibitem{rr15}X. Zhang, S. Boccaletti, S. Guan, and Z. Liu, \textit{Explosive synchronization in adaptive and multilayer networks}, Phys. Rev. Lett. \textbf{114}, 038701 (2015).
\bibitem{rr16}J. Miake, E. Marban, H. B. Nuss, \textit{Biological pacemaker created by gene transfer}, Nature \textbf{419}, 132-133 (2002).
\bibitem{rr17} J. Jalife, R. A. Gray, G. E. Morley, J. M. Davidenko, \textit{Self-organization and the dynamical nature of ventricular fibrillation}, Chaos \textbf{8}, 79-93 (1998).
\bibitem{rr18} P. J. Menck, J. Heitzig, J. Kurths, H. J. Schellnhuber, \textit{How dead ends undermine power grid stability}, Nat.
Commun. \textbf{5}, 3969 (2014).
\end{thebibliography}


